Formation of Quasi-Singularities for Compressible Euler Flows

This paper establishes a novel quasi-singularity formation phenomenon for the three-dimensional isentropic compressible Euler equations. For any prescribed finite collections of pairwise distinct points $\{z^{(1)}_j\}_{j=1}^N, \{z^{(2)}_j\}_{j=1}^N \subset \mathbb{R}^3$, an arbitrarily large parameter $M \gg 1$, and an arbitrary time $T>0$, we explicitly construct real-analytic initial data and an external force generated by Herglotz-type wave fields together with a suitably chosen damping parameter. We prove that the corresponding unique classical solution exists on $[0,T]$ and exhibits the following properties: first, the pressure remains uniformly bounded from below and above proportionally to the constant initial pressure; second, every component of the velocity and its first-order spatial derivatives simultaneously undergo high-amplitude (exceeding $M$) and high-frequency oscillations at all points $z^{(1)}_j$ ($j=1,\dots,N$) throughout $[0,T]$; and third, the velocity and its first-order spatial derivatives remain uniformly bounded by $1$ at all points $z^{(2)}_j$ ($j=1,\dots,N$) throughout $[0,T]$. The construction exhibits two complementary features: localized large-amplitude oscillations of the velocity and its spatial gradient at prescribed points, and a pronounced contrast between the two groups of points. Since the solution remains smooth, this behavior may be viewed as an intermediate regime between moderate regular flows and genuine finite-time blowup. Moreover, the initial data, external force, and damping parameter are specified explicitly, providing a concrete framework for investigating such behavior in controlled compressible flows. The proof combines the construction of Herglotz wave fields with a suitable choice of the damping parameter and quantitative energy estimates for the nonlinear remainder.

==> focused_numerics_section.tex <==
\section{Numerical experiment on velocity and gradient contrast}
\label{sec:numerical-contrast}

We measure the velocity and its first spatial derivatives at the
four prescribed points. The objective is a large oscillation in
the first group and a small response in the second. The diagnostics
are based on the computed solution $v$ and its gradient.

\subsection{Geometry and initial data}
We set $M=10$, $T=10$, and
\[
 (z_1^{(1)},z_2^{(1)})=((0,0,0),(0,0,1)),\qquad
 (z_1^{(2)},z_2^{(2)})=((1,0,1),(1,0,0)).
\]
Take $\gamma=7/5$ and choose the pressure-law constant $A$ so that
$\omega_0=10^3$. The resulting parameters are
\[
 p_0=M^{2\gamma/(\gamma-1)}=10^7,\qquad
 A=\left(\frac{\omega_0^2}{\gamma M^2}\right)^\gamma,
 \qquad \rho_0=\frac{\gamma p_0}{\omega_0^2}=14.
\]
The target period $2\pi/\omega_0$ is approximately $0.006283$.
There are $1591$ complete target cycles in $[0,10]$.

The whole-space initial data of Theorem~\ref{thm:quasi-singularity}
are $p(0,x)=10^7$ and $v(0,x)=\nabla H_g(x)$. To specify $H_g$ for
these four points, order the points as
$(z_1^{(1)},z_2^{(1)},z_1^{(2)},z_2^{(2)})$ and use the nine
multi-indices
\[
 \mathcal J=(0,e_1,e_2,e_3,2e_1,e_1+e_2,e_1+e_3,2e_2,e_2+e_3).
\]
The jet vector $C$ has two consecutive copies of each of the blocks
\[
 \begin{aligned}
 c^{(1)}&=(-33,11,11,11,11,11,11,11,11),\\
 c^{(2)}&=(-3/2,1/2,1/2,1/2,1/2,1/2,1/2,1/2,1/2).
 \end{aligned}
\]
These are the entries in the Herglotz construction of
Corollary~\ref{thm:acoustic-profile}. The unlisted diagonal entry
$\partial_{x_3 x_3}^2 H_g$ follows from $\Delta H_g=-H_g$.

For the computation, we use $24$ Gauss--Legendre nodes in the polar
cosine and $48$ equally spaced azimuthal nodes. Let $(d_\ell,w_\ell)$,
$1\leq\ell\leq1152$, denote the resulting sphere directions and
weights. The coefficients $a_\ell$ form the minimum Euclidean norm
solution of the linear system $Ba=C$, where
\[
 B_{(j,\beta),\ell}
   =\sqrt{w_\ell}(\mathrm i d_\ell)^\beta
      \exp(\mathrm i z_j\cdot d_\ell),\qquad \beta\in\mathcal J.
\]
We compute $a$ by singular value decomposition. The maximum residual
in the prescribed jet entries is below $2\times10^{-10}$.
The velocity initial data used on the numerical box are therefore
\begin{equation}\label{eq:experiment-initial-data}
 \begin{aligned}
 p(0,x)&=10^7,\\
 v(0,x)&=\chi_b(x)\operatorname{Re}
       \sum_{\ell=1}^{1152}
       \mathrm i\,d_\ell\sqrt{w_\ell}\,a_\ell
       \exp(\mathrm i x\cdot d_\ell).
 \end{aligned}
\end{equation}
Here $b=0.25$ and the periodic box is
$\Omega_b=[-b,1+b]\times[-b,b]\times[-b,1+b]$.
The product cutoff $\chi_b$ is one on a neighborhood of the
probes and vanishes to all orders at the box boundary. Its
factors start to decrease at distance $0.145$ from the
interval $[0,1]$ in the $x_1,x_3$ directions and from $\{0\}$
in the $x_2$ direction. In the transition region a factor is
$(1+\exp((1-s)^{-1}-s^{-1}))^{-1}$, where
$s$ is the distance beyond $0.145$ divided by $b-0.145$.
We set $v_h(t,x)=v(0,x)\cos(\omega_0 t)$ and
$f(t,x)=\kappa v_h(t,x)$.

\subsection{Choice of damping and pointwise diagnostics}
We compare only $\kappa=10^6$ and $\kappa=10^7$. Both are large
relative to the target angular frequency, with
$\kappa/\omega_0=10^3$ and $10^4$, respectively. The sufficient
coefficient in Theorem~\ref{thm:quasi-singularity} takes the form
\[
 K_*(1+T)M^2\exp(K_*MT)=1100K_*\exp(100K_*)
\]
for the present parameters. The theorem chooses $K_*$ in a
uniform energy estimate. We choose the two numerical coefficients
by testing the velocity and gradient at the four probes in the
periodic computation.

With $r=\rho/\rho_0$ and $w=v-v_h$, the numerical equations are
\[
 \begin{aligned}
 \partial_t r &=-\operatorname{div}(rv),\\
 \partial_t w+\kappa w
 &=-\partial_t v_h-v\cdot\nabla v
   -\omega_0^2 r^{\gamma-2}\nabla r,\qquad
 v=v_h+w.
 \end{aligned}
\]
We use the same $60\times20\times60$ periodic grid, with
spacing $h=0.025$, in both runs. Fourth-order centered finite
differences are applied to the mass flux and the spatial
derivatives. We treat the linear relaxation in the exponential
Runge--Kutta method of Cox and Matthews~\cite{CoxMatthews2002ETD}.
The steps are $\Delta t=10/128000$ for $\kappa=10^6$ and
$\Delta t=10/40000$ for $\kappa=10^7$. The computed gradient
combines the analytic derivative of $v_h$ on the box with the
finite-difference derivative of $w$.

Write $F$ for either $v$ or $\nabla v$ and $F_a$ for its scalar
entries. The theorem compares signed values in the first group
at the target peak times $t_m=m\pi/\omega_0$ and absolute values
in the second group on the entire time interval. To make the
amplitude comparison independent of the precise peak times, we
also compute sampled peaks in the intervals
\[
 I_m=\left[t_m-\frac{\pi}{2\omega_0},
            t_m+\frac{\pi}{2\omega_0}\right]\cap[0,T].
\]
For each $m$ we select, in the first group, the time sample
that maximizes the simultaneous signed lower bound
\[
 \max_{t_n\in I_m}\min_{j,a}
       (-1)^m F_a(t_n,z_j^{(1)}).
\]
For the second group we take $\max_{t_n\in I_m,j,a}
|F_a(t_n,z_j^{(2)})|$. Figure~\ref{fig:focused-all-peaks}
places these values at their respective time samples. We also
evaluate the simultaneous signed bound at each exact target
time $t_m$ using cubic time interpolation, and report its
minimum in Table~\ref{tab:focused-damping}.

\subsection{Time traces and observed peak contrast}
Figures~\ref{fig:focused-velocity-windows} and
\ref{fig:focused-gradient-windows} show the computed
$v^{(1)}$ and $\partial_{x_1}v^{(1)}$ during three windows:
near the start, around $t=5$, and near $t=10$. For each
quantity, the first and second probe within a group are
distinguished by their line styles. The same colors identify
the two damping strengths throughout the section.

\begin{table}[tbp]
 \centering
 \small
 \caption{Velocity and gradient diagnostics over $[0,10]$ on the
 $h=0.025$ grid. The first-group entries are minima of the signed
 components at the prescribed peak times. The second-group
 entries are maxima of absolute components over all saved times.}
 \label{tab:focused-damping}
 \begin{tabular}{crrrr}
 \toprule
 & \multicolumn{2}{c}{First group}
 & \multicolumn{2}{c}{Second group}\\
 $\kappa$ & Velocity & Gradient & Velocity & Gradient\\
 \midrule
 $10^6$ & 10.9346 & 1.0588 & 0.7848 & 8.8669\\
 $10^7$ & 10.9835 & 10.7640 & 0.5098 & 0.7479\\
 \bottomrule
 \end{tabular}
\end{table}

For $\kappa=10^6$, all velocity entries in the first group attain the prescribed sign and exceed $10$ in signed value at each target peak. The largest sampled absolute velocity entry in the second group is \(0.7848\). The second-group gradient maximum is \(8.8669\), which exceeds the threshold $1$.

For $\kappa=10^7$, both the velocity and the gradient meet the first-group peak thresholds and the second-group bounds in the numerical diagnostics. The respective second-group maxima are \(0.5098\) and \(0.7479\).

The smallest common sampled velocity peaks over the half-cycles are \(10.9281\) and \(10.8984\), respectively.

In the previous resolution check for $\kappa=10^6$, the
$h=0.0125$ mesh on $[0,0.0125]$ gave second-group maxima
of approximately $0.791$ for velocity and $7.635$ for gradient.
For $\kappa=10^7$, halving the time step and increasing the box
padding to $0.30$ in two separate runs gave second-group gradient
maxima of $0.745$ and $0.568$, respectively. These tests indicate
that the threshold comparisons persist in the tested
discretizations, with sensitivity of individual gradient
magnitudes to mesh and box size.

\begin{figure}[tbp]
 \centering
 \includegraphics[width=\linewidth]{figures/velocity_time_windows.pdf}
 \caption{Computed velocity component $v^{(1)}$ at each probe in
 three time windows. Solid and dashed curves distinguish the
 first and second probes within each group, respectively. Dotted
 horizontal lines mark $\pm10$ in the first group and $\pm1$
 in the second.}
 \label{fig:focused-velocity-windows}
\end{figure}

\begin{figure}[tbp]
 \centering
 \includegraphics[width=\linewidth]{figures/gradient_time_windows.pdf}
 \caption{Computed derivative $\partial_{x_1}v^{(1)}$ at the
 four probes. The colors, line styles, and thresholds match
 Figure~\ref{fig:focused-velocity-windows}.}
 \label{fig:focused-gradient-windows}
\end{figure}

\begin{figure}[tbp]
 \centering
 \includegraphics[width=\linewidth]{figures/all_half_cycle_peaks.pdf}
 \caption{Computed peaks over all half-cycles in $[0,10]$.
 The top panels use all velocity components and the bottom panels
 use all gradient entries. On the left, each value is the largest
 simultaneous signed lower bound found among the samples in its
 half-cycle. On the right, each value is the largest sampled
 absolute entry within its half-cycle.}
 \label{fig:focused-all-peaks}
\end{figure}

\clearpage
\subsection{Spatial contrast near the probes}
Figures~\ref{fig:focused-spatial-early},
\ref{fig:focused-spatial-middle}, and~\ref{fig:focused-spatial-late}
show neighborhoods of the four probes in the plane $x_2=0$ at
one early, one middle, and one late target peak. The same
physical times are used for the two damping strengths. Figure~\ref{fig:focused-spatial-actual}
shows the corresponding fields at the sampled common velocity
crest in the early half-cycle for each coefficient.
For each snapshot we interpolate $w$ linearly in time between
adjacent states and evaluate $v_h$ at the specified time.
The color represents $\max_i |v^{(i)}|$ or
$\max_{i,j}|\partial_{x_j}v^{(i)}|$. Darker shades represent larger
values, and the scale for each quantity is fixed across all
figures. The numbers in the panels give the value
at the center probe. The spatial fields can vary rapidly
outside the marked points, where the probe thresholds do not
apply.

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=0.94\linewidth]{figures/spatial_peaks_m32.pdf}
 \caption{Spatial magnitudes in the early window at
 $t_{32}\simeq0.10053$. The upper two rows show velocity and
 the lower two show the first spatial derivatives.}
 \label{fig:focused-spatial-early}
\end{figure}

\begin{figure}[p]
 \centering
 \includegraphics[width=\linewidth]{figures/spatial_peaks_m1591.pdf}
 \caption{Spatial magnitudes near the middle of the interval at
 $t_{1591}\simeq4.99827$, a negative peak of the target.}
 \label{fig:focused-spatial-middle}
\end{figure}

\begin{figure}[p]
 \centering
 \includegraphics[width=\linewidth]{figures/spatial_peaks_m3180.pdf}
 \caption{Spatial magnitudes near the end of the interval at
 $t_{3180}\simeq9.99026$. The color scales agree with
 Figures~\ref{fig:focused-spatial-early} and
 \ref{fig:focused-spatial-middle}.}
 \label{fig:focused-spatial-late}
\end{figure}


\begin{figure}[p]
 \centering
 \includegraphics[width=\linewidth]{figures/spatial_actual_velocity_crests.pdf}
 \caption{Spatial magnitudes at the sampled common velocity crest
 within $I_{32}$ for each damping coefficient. The crest time is
 chosen from the computed velocities in the first group. Both
 quantities use the same color scales as the prescribed-phase
 snapshots.}
 \label{fig:focused-spatial-actual}
\end{figure}


==> focused_section_template.tex <==
\section{Numerical experiment on velocity and gradient contrast}
\label{sec:numerical-contrast}

We measure the velocity and its first spatial derivatives at the
four prescribed points. The objective is a large oscillation in
the first group and a small response in the second. The diagnostics
are based on the computed solution $v$ and its gradient.

\subsection{Geometry and initial data}
We set $M=10$, $T=10$, and
\[
 (z_1^{(1)},z_2^{(1)})=((0,0,0),(0,0,1)),\qquad
 (z_1^{(2)},z_2^{(2)})=((1,0,1),(1,0,0)).
\]
Take $\gamma=7/5$ and choose the pressure-law constant $A$ so that
$\omega_0=10^3$. The resulting parameters are
\[
 p_0=M^{2\gamma/(\gamma-1)}=10^7,\qquad
 A=\left(\frac{\omega_0^2}{\gamma M^2}\right)^\gamma,
 \qquad \rho_0=\frac{\gamma p_0}{\omega_0^2}=14.
\]
The target period $2\pi/\omega_0$ is approximately $0.006283$.
There are $1591$ complete target cycles in $[0,10]$.

The whole-space initial data of Theorem~\ref{thm:quasi-singularity}
are $p(0,x)=10^7$ and $v(0,x)=\nabla H_g(x)$. To specify $H_g$ for
these four points, order the points as
$(z_1^{(1)},z_2^{(1)},z_1^{(2)},z_2^{(2)})$ and use the nine
multi-indices
\[
 \mathcal J=(0,e_1,e_2,e_3,2e_1,e_1+e_2,e_1+e_3,2e_2,e_2+e_3).
\]
The jet vector $C$ has two consecutive copies of each of the blocks
\[
 \begin{aligned}
 c^{(1)}&=(-33,11,11,11,11,11,11,11,11),\\
 c^{(2)}&=(-3/2,1/2,1/2,1/2,1/2,1/2,1/2,1/2,1/2).
 \end{aligned}
\]
These are the entries in the Herglotz construction of
Corollary~\ref{thm:acoustic-profile}. The unlisted diagonal entry
$\partial_{x_3 x_3}^2 H_g$ follows from $\Delta H_g=-H_g$.

For the computation, we use $24$ Gauss--Legendre nodes in the polar
cosine and $48$ equally spaced azimuthal nodes. Let $(d_\ell,w_\ell)$,
$1\leq\ell\leq1152$, denote the resulting sphere directions and
weights. The coefficients $a_\ell$ form the minimum Euclidean norm
solution of the linear system $Ba=C$, where
\[
 B_{(j,\beta),\ell}
   =\sqrt{w_\ell}(\mathrm i d_\ell)^\beta
      \exp(\mathrm i z_j\cdot d_\ell),\qquad \beta\in\mathcal J.
\]
We compute $a$ by singular value decomposition. The maximum residual
in the prescribed jet entries is below $2\times10^{-10}$.
The velocity initial data used on the numerical box are therefore
\begin{equation}\label{eq:experiment-initial-data}
 \begin{aligned}
 p(0,x)&=10^7,\\
 v(0,x)&=\chi_b(x)\operatorname{Re}
       \sum_{\ell=1}^{1152}
       \mathrm i\,d_\ell\sqrt{w_\ell}\,a_\ell
       \exp(\mathrm i x\cdot d_\ell).
 \end{aligned}
\end{equation}
Here $b=0.25$ and the periodic box is
$\Omega_b=[-b,1+b]\times[-b,b]\times[-b,1+b]$.
The product cutoff $\chi_b$ is one on a neighborhood of the
probes and vanishes to all orders at the box boundary. Its
factors start to decrease at distance $0.145$ from the
interval $[0,1]$ in the $x_1,x_3$ directions and from $\{0\}$
in the $x_2$ direction. In the transition region a factor is
$(1+\exp((1-s)^{-1}-s^{-1}))^{-1}$, where
$s$ is the distance beyond $0.145$ divided by $b-0.145$.
We set $v_h(t,x)=v(0,x)\cos(\omega_0 t)$ and
$f(t,x)=\kappa v_h(t,x)$.

\subsection{Choice of damping and pointwise diagnostics}
We compare only $\kappa=10^6$ and $\kappa=10^7$. Both are large
relative to the target angular frequency, with
$\kappa/\omega_0=10^3$ and $10^4$, respectively. The sufficient
coefficient in Theorem~\ref{thm:quasi-singularity} takes the form
\[
 K_*(1+T)M^2\exp(K_*MT)=1100K_*\exp(100K_*)
\]
for the present parameters. The theorem chooses $K_*$ in a
uniform energy estimate. We choose the two numerical coefficients
by testing the velocity and gradient at the four probes in the
periodic computation.

With $r=\rho/\rho_0$ and $w=v-v_h$, the numerical equations are
\[
 \begin{aligned}
 \partial_t r &=-\operatorname{div}(rv),\\
 \partial_t w+\kappa w
 &=-\partial_t v_h-v\cdot\nabla v
   -\omega_0^2 r^{\gamma-2}\nabla r,\qquad
 v=v_h+w.
 \end{aligned}
\]
We use the same $60\times20\times60$ periodic grid, with
spacing $h=0.025$, in both runs. Fourth-order centered finite
differences are applied to the mass flux and the spatial
derivatives. We treat the linear relaxation in the exponential
Runge--Kutta method of Cox and Matthews~\cite{CoxMatthews2002ETD}.
The steps are $\Delta t=10/128000$ for $\kappa=10^6$ and
$\Delta t=10/40000$ for $\kappa=10^7$. The computed gradient
combines the analytic derivative of $v_h$ on the box with the
finite-difference derivative of $w$.

Write $F$ for either $v$ or $\nabla v$ and $F_a$ for its scalar
entries. The theorem compares signed values in the first group
at the target peak times $t_m=m\pi/\omega_0$ and absolute values
in the second group on the entire time interval. To make the
amplitude comparison independent of the precise peak times, we
also compute sampled peaks in the intervals
\[
 I_m=\left[t_m-\frac{\pi}{2\omega_0},
            t_m+\frac{\pi}{2\omega_0}\right]\cap[0,T].
\]
For each $m$ we select, in the first group, the time sample
that maximizes the simultaneous signed lower bound
\[
 \max_{t_n\in I_m}\min_{j,a}
       (-1)^m F_a(t_n,z_j^{(1)}).
\]
For the second group we take $\max_{t_n\in I_m,j,a}
|F_a(t_n,z_j^{(2)})|$. Figure~\ref{fig:focused-all-peaks}
places these values at their respective time samples. We also
evaluate the simultaneous signed bound at each exact target
time $t_m$ using cubic time interpolation, and report its
minimum in Table~\ref{tab:focused-damping}.

\subsection{Time traces and observed peak contrast}
Figures~\ref{fig:focused-velocity-windows} and
\ref{fig:focused-gradient-windows} show the computed
$v^{(1)}$ and $\partial_{x_1}v^{(1)}$ during three windows:
near the start, around $t=5$, and near $t=10$. For each
quantity, the first and second probe within a group are
distinguished by their line styles. The same colors identify
the two damping strengths throughout the section.

\begin{table}[tbp]
 \centering
 \small
 \caption{Velocity and gradient diagnostics over $[0,10]$ on the
 $h=0.025$ grid. The first-group entries are minima of the signed
 components at the prescribed peak times. The second-group
 entries are maxima of absolute components over all saved times.}
 \label{tab:focused-damping}
 \begin{tabular}{crrrr}
 \toprule
 & \multicolumn{2}{c}{First group}
 & \multicolumn{2}{c}{Second group}\\
 $\kappa$ & Velocity & Gradient & Velocity & Gradient\\
 \midrule
 @ROWS@
 \bottomrule
 \end{tabular}
\end{table}

@INTERPRETATION@

In the previous resolution check for $\kappa=10^6$, the
$h=0.0125$ mesh on $[0,0.0125]$ gave second-group maxima
of approximately $0.791$ for velocity and $7.635$ for gradient.
For $\kappa=10^7$, halving the time step and increasing the box
padding to $0.30$ in two separate runs gave second-group gradient
maxima of $0.745$ and $0.568$, respectively. These tests indicate
that the threshold comparisons persist in the tested
discretizations, with sensitivity of individual gradient
magnitudes to mesh and box size.

\begin{figure}[tbp]
 \centering
 \includegraphics[width=\linewidth]{figures/velocity_time_windows.pdf}
 \caption{Computed velocity component $v^{(1)}$ at each probe in
 three time windows. Solid and dashed curves distinguish the
 first and second probes within each group, respectively. Dotted
 horizontal lines mark $\pm10$ in the first group and $\pm1$
 in the second.}
 \label{fig:focused-velocity-windows}
\end{figure}

\begin{figure}[tbp]
 \centering
 \includegraphics[width=\linewidth]{figures/gradient_time_windows.pdf}
 \caption{Computed derivative $\partial_{x_1}v^{(1)}$ at the
 four probes. The colors, line styles, and thresholds match
 Figure~\ref{fig:focused-velocity-windows}.}
 \label{fig:focused-gradient-windows}
\end{figure}

\begin{figure}[tbp]
 \centering
 \includegraphics[width=\linewidth]{figures/all_half_cycle_peaks.pdf}
 \caption{Computed peaks over all half-cycles in $[0,10]$.
 The top panels use all velocity components and the bottom panels
 use all gradient entries. On the left, each value is the largest
 simultaneous signed lower bound found among the samples in its
 half-cycle. On the right, each value is the largest sampled
 absolute entry within its half-cycle.}
 \label{fig:focused-all-peaks}
\end{figure}

\clearpage
\subsection{Spatial contrast near the probes}
Figures~\ref{fig:focused-spatial-early},
\ref{fig:focused-spatial-middle}, and~\ref{fig:focused-spatial-late}
show neighborhoods of the four probes in the plane $x_2=0$ at
one early, one middle, and one late target peak. The same
physical times are used for the two damping strengths. Figure~\ref{fig:focused-spatial-actual}
shows the corresponding fields at the sampled common velocity
crest in the early half-cycle for each coefficient.
For each snapshot we interpolate $w$ linearly in time between
adjacent states and evaluate $v_h$ at the specified time.
The color represents $\max_i |v^{(i)}|$ or
$\max_{i,j}|\partial_{x_j}v^{(i)}|$. Darker shades represent larger
values, and the scale for each quantity is fixed across all
figures. The numbers in the panels give the value
at the center probe. The spatial fields can vary rapidly
outside the marked points, where the probe thresholds do not
apply.

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=0.94\linewidth]{figures/spatial_peaks_m32.pdf}
 \caption{Spatial magnitudes in the early window at
 $t_{32}\simeq0.10053$. The upper two rows show velocity and
 the lower two show the first spatial derivatives.}
 \label{fig:focused-spatial-early}
\end{figure}

\begin{figure}[p]
 \centering
 \includegraphics[width=\linewidth]{figures/spatial_peaks_m1591.pdf}
 \caption{Spatial magnitudes near the middle of the interval at
 $t_{1591}\simeq4.99827$, a negative peak of the target.}
 \label{fig:focused-spatial-middle}
\end{figure}

\begin{figure}[p]
 \centering
 \includegraphics[width=\linewidth]{figures/spatial_peaks_m3180.pdf}
 \caption{Spatial magnitudes near the end of the interval at
 $t_{3180}\simeq9.99026$. The color scales agree with
 Figures~\ref{fig:focused-spatial-early} and
 \ref{fig:focused-spatial-middle}.}
 \label{fig:focused-spatial-late}
\end{figure}


\begin{figure}[p]
 \centering
 \includegraphics[width=\linewidth]{figures/spatial_actual_velocity_crests.pdf}
 \caption{Spatial magnitudes at the sampled common velocity crest
 within $I_{32}$ for each damping coefficient. The crest time is
 chosen from the computed velocities in the first group. Both
 quantities use the same color scales as the prescribed-phase
 snapshots.}
 \label{fig:focused-spatial-actual}
\end{figure}

